Learning Deep Object Detectors from 3D Models

Crowdsourced 3D CAD models are becoming easily accessible online, and can potentially generate an infinite number of training images for almost any object category.We show that augmenting the training data of contemporary Deep Convolutional Neural Net (DCNN) models with such synthetic data can be effective, especially when real training data is limited or not well matched to the target domain. Most freely available CAD models capture 3D shape but are often missing other low level cues, such as realistic object texture, pose, or background. In a detailed analysis, we use synthetic CAD-rendered images to probe the ability of DCNN to learn without these cues, with surprising findings. In particular, we show that when the DCNN is fine-tuned on the target detection task, it exhibits a large degree of invariance to missing low-level cues, but, when pretrained on generic ImageNet classification, it learns better when the low-level cues are simulated. We show that our synthetic DCNN training approach significantly outperforms previous methods on the PASCAL VOC2007 dataset when learning in the few-shot scenario and improves performance in a domain shift scenario on the Office benchmark.

==> approach.tex <==
\section{Exploring the Invariances of CNN features}
\label{approach}

In this section, we design an experimental paradigm to evaluate how variations in image formation factors affect the deep representation learned by the CNN. The main idea is to train classifiers on synthetic data using the network's hidden layer activations as the feature representation, and test their performance on real image data.

Specifically, for each experiment, we follow these steps
 (see Figure~\ref{fig:overview}): 1) select image formation parameters, 2) generate a batch of synthetic 2D images with those parameters, 3) sample positive and negative patches for each class, 4) extract hidden CNN layer activations from the patches as features, 5) train a classifier for each object category, 6) test the classifiers on real images.

We base our approach on the intuition that, if the network has learned to be invariant to a certain factor, then similar neurons will activate, whether or not that factor is present in the input image. For example, if the network is invariant to ``cat'' texture, then it will have similar activations on cats with and without texture, i.e. it will ``hallucinate'' the right texture when given a texureless cat shape. Then the classifier will learn equally well from both sets of training data. If, on the other hand, the network is not invariant to texture, then the feature distributions will differ. As a consequence, the classifier trained on textureless cat data will perform worse than the classifier trained on both shape and texture.

%We evaluate invariance in two ways: \kate{by visualizing the activations??} and by testing the classifiers on real image data. 

%\kate{any reason for testing only on real and not synthetic data?} \kate{add figure with visualization of activations}

\subsection{CNN Model and Training}

We adopt the detection method of~\cite{RCNN}, which uses the eight-layer ``AlexNet'' architecture with over 60 million parameters~\cite{alexnet}. This network had first achieved breakthrough results on the ILSVRC-2012~\cite{ilsvrc2012} image classification, and remains the most studied and widely used visual convnet.
The network is trained by fully supervised back-propagation (as in~\cite{lecun89}) and takes raw RGB image pixels of a fixed size of 224 $\times$ 224 and outputs object category labels.
%Each layer consists of a set of neurons, each with linear weights on the input followed by a nonlinearity. 
The first five layers of the network have local spatial support and are convolutional, while the final three layers are fully-connected to each neuron from the previous layer, and thus include inputs from the entire image. 

This network, originally designed for classification, was applied and fine-tuned to detection in~\cite{RCNN} with impressive gains on the popular object detction benchmarks. To adapt AlexNet for detection, the RCNN applied the network to each image sub-region proposed by the Selective Search method (\cite{selective-search}), adding a background label, and applied non-maximal suppression to the outputs. Fine-tuning all hidden layers resulted in performance improvements. We refer the reader to~\cite{RCNN} for more details. 

Our hypothesis is that the network will learn different invariances, depending on how it is trained. Therefore, we evaluate two different variants of the network: one trained on the ImageNet ILSVRC 1000-way classification task, which we call {\small IMGNET}, and the same network also fine-tuned for the PASCAL detection task, which we call {\small PASC-FT}. For both networks, we extract the last hidden layer (fc7) as the feature representation. We choose to focus on the last hidden layer as it is the most high-level representation and has learned the most invariance.

%\subsection{Image Formation Factors}
\subsection{Synthetic Data Generation}

Object appearance is altered by many image formation factors, including object shape, pose, surface color, reflectance, location and spectral distributions of illumination sources, properties of the background scene, camera characteristics, etc. We choose a subset of factors that can easily be modeled using simple computer graphics techniques, namely, \textbf{object texture} and \textbf{color}, \textbf{context/background} appearance and color, \textbf{3D pose} and \textbf{3D shape}. We study the invariance of the CNN representation to these parameters using synthetic data.  We also study the invariance to 3D rigid rotations using real data. The difference in treatment (using both synthetic and real data for pose) stems from the fact that while we can readily control for variations in 3D rigid rotations by making appropriate selections from existing datasets, the same cannot be said for object texture, color, shape and background appearance. 

%In what follows, we describe our overall procedure for generating 2D training images from 3D CAD models, and discuss our experiments aimed at elucidating the CNN's invariance to our selected subset of image formation factors.

We downloaded CAD models from 3D Warehouse by searching for the name of $20$ object categories represented in the PASCAL VOC Dataset. For each category, around $25$ models were downloaded. We explore the effect of intra-class shape variation by restricting the number of models below.
%\kate{any manual cleanup??} \xpeng{No}\kate{show examples in figure}\kate{explain the experiment varying the number of shapes} 
The original poses of the CAD models can be arbitrary (ex. upside-down chairs, or tilted cars). We therefore adjust the CAD models's viewpoint manually to $3$ or $4$ ``views''(as shown in Figure \ref{fig:overview}) %\kate{Are these same as Fig2?if so, refer to figure} 
that best represent intra-class pose variance for PASCAL objects. Next, for each manually specified model view, we generate several small perturbations by adding a random rotation. 
%$1$ or $2$ 
Finally, for each pose variation, we select the texture, color and background image and render a virtual image to include in our virtual training dataset. 
Next, we describe the detailed process for each factor, and present results.

%The final number of images in the virtual training dataset is $2000$, with $100$ positive instances per each of the $20$ categories.
%The procedure for rendering 2D images from 3D CAD models is identical to that of~\cite{BMVC}.

\subsection{Object Color, Texture and Context}

We begin by investigating various combination of object colors and textures placed against a variety of background scene colors and textures. Previous work by~\cite{BMVC} has shown that when training a HOG model from virtual data, rendering natural backgrounds and texture is not helpful. The intuition is that a HOG-based classifier is focused on learning the ``outlines'' of the object shape. We hypothesise that the case is different for CNN representations, where certain neurons have been shown to respond to textures, colors and other mid-level patterns.

We examine the invariance of the CNN representation to two types of object textures, namely realistic color textures, and uniform grayscale textures (i.e., no texture at all). In the case of background scenes, we examine invariance to three types of scenes, namely real-image color scenes, real-image grayscale scenes, and a plain white background. Examples of our texture and background generation settings are shown in Table~\ref{tab:color}. 

%\subsubsection{Experimental setup}

In order to simulate realistic object textures, we gathered $5$ to $8$ real images (per category) containing real objects and extracted the textures therein by annotating a bounding box. Then the texture images will be stretched to fit the CAD models. Likewise, in order to simulate realistic background scenes, we gathered about 40 (per category) real images of scenes where each category is likely to appear (e.g blue sky images for aeroplane, images of a lake or ocean for boat, etc.). When generating a virtual image, we first randomly select a background image from the available background pool and project it onto the image plane. Then, we select a random texture image from the texture pool and map it onto the CAD model before rendering the object.
For this experiment, we used 1-2 pose perturbations per view and all views per category. The final number of images in the virtual training dataset is $2000$, with $100$ positive instances per each of the $20$ categories.

We trained a series of detectors with each of the above background and object texture configurations and tested them on the PASCAL VOC test set, reporting the average precision (AP) across categories.
Results are shown in Table~\ref{tab:color}. As expected, we see that training with synthetic data obtains lower mean AP than training with real data (around 58\% with bounding box regression). Also, the IMGNET network representation achieves lower performance than the PASC-FT network, as was the case for real data in ~\cite{RCNN}. However, the somewhat unexpected result is that the generation settings \textbf{RR-RR, W-RR, W-UG, RG-RR} with PASC-FT all achieve comparable performance, despite the fact that \textbf{W-UG} has no texture and no context. Results with real texture but no color in the background (\textbf{RG-RR, W-RR}) are the best. This indicates that the network has learned to be invariant to the color and texture of the object and its background. Also, we note that settings \textbf{RR-UG} and \textbf{RG-UG} achieve much lower performance (6-9 points lower), potentially because the uniform texture is not well distinguished from either real color or real grayscale backgrounds. 

%is determined by how distinguished the object is from the background. When using W-UG, the mAP-30.14\% is comparable to the mAP-28.9\% from VCNN trained by virtual images with RR-RR. And when using the  RG-RR on the target objects, the mAP is 31.18\%, 6-9 points higher than the performance of VCNN trained on virtual images with RR-UG and VCNN trained on virtual images with RG-UG, in which the foreground images are not quite distinguished from the background.

For the IMGNET network, the trend is similar, but with the best performing methods being \textbf{RR-RR} and \textbf{RG-RR}. This means that adding realistic context and texture statistics helps the classifier, and thus the IMGNET network is somewhat less invariant to these factor, at least for the categories in our dataset. We note that the IMGNET network has seen these categories in training, as they are part of the ILSVRC 1000-way classification task, which explains why it is still fairly insensitive. Combinations of uniform texture with a real background also do not perform well here. Interestingly, \textbf{RG-RR} does very well with both networks, leading to the conclusion that both networks have learned to associate the right context colors with objects.

%REMINDER: fix the first row of the IMGNET table to include RR-RR dataset #1

\begin{table*}[t]
\scriptsize  
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|}
\hline
 &\textbf {RR-RR} & \textbf{W-RR}&\textbf{W-UG}  &\textbf{RR-UG}&\textbf{RG-UG}&\textbf{RG-RR}\\ 
\hline
\footnotesize{BG} & Real RGB&White & White &Real RGB&Real Gray&Real Gray\\
\hline
\footnotesize{TX} &Real RGB & Real RGB&Unif. Gray&Unif. Gray&Unif. Gray&Real RGB\\
\hline
%
& \includegraphics[width=0.7in]{real_real.jpg}
&\includegraphics[width=0.7in]{white_real.jpg}
& \includegraphics[width=0.7in]{white_gray.jpg}
&\includegraphics[width=0.7in]{real_gray.jpg}
&\includegraphics[width=0.7in]{realgray_gray.jpg}
&\includegraphics[width=0.7in]{realgray_real.jpg}\\
%
\hline
\end{tabular}
%
\begin{tabular}
%{c|| c c}
{ c  ||  p{0.15cm}  p{0.15cm}  p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.25cm}|p{0.15cm}}
%\textbf{VOC 2007}
\textsc{PASC-FT}
 &aero& bike&bird&boat&botl	&bus&car&cat&chr	&cow	&tab	&dog	&hse	&mbik	&pers	&plt	&shp	&sofa	&trn	&tv&mAP\\

%\textbf{RCNN-fc7}&64.2&69.7&41.9&	32&	62.6&	71&	60.7&	32.7&	58.5&	46.5&	56.1&	60.6&	66.8&	54.2&	31.5&	52.8&	48.9&	57.9&	64.7&	51.665\\
\hline
\textbf{RR-RR}&50.9 &57.5 &28.3 &20.3 &17.8 &50.1 &37.7 &26.1 &11.5 &27.1 &2.4 &25.3 &40.2 &52.2 &14.3 &11.9 &40.4 &16.3 &15.2 &32.2 &28.9 \\
\textbf{W-RR} &46.5 &55.8 &28.6 &21.7 &21.3 &50.6 &46.6 &28.9 &14.9 &38.1 &0.7 &27.3 &42.5 &53.0 &17.4 &22.8 &30.4 &16.4 &16.7 &43.5 &31.2 \\
\textbf{W-UG}&54.4 &49.6 &31.5 &24.8 &27.0 &42.3 &62.9 &6.6 &21.2 &34.6 &0.3 &18.2 &35.4 &51.3 &33.9 &15.0 &8.3 &33.9 &2.6 &49.0 &30.1\\
\textbf{RR-UG}&55.2 &57.8 &24.8 &17.1 &11.5 &29.9 &39.3 &16.9 &9.9 &35.1 &4.7 &30.1 &37.5 &53.1 &18.1 &9.5 &12.4 &18.2 &2.1 &21.1 &25.2 \\
\textbf{RG-UG}&49.8 &56.9 &20.9 &15.6 &10.8 &25.6 &42.1 &14.7 &4.1 &32.4 &9.3 &20.4 &28.0 &51.2 &14.7 &10.3 &12.6 &14.2 &9.5 &28.0 &23.6 \\
\textbf{RG-RR}&46.5&55.8&28.6&21.7&21.3&50.6&46.6&28.9&14.9&38.1&0.7&27.3&42.5&53.0&17.4&22.8&30.4&16.4&16.7&43.5&31.2\\
\hline
\end{tabular}

\begin{tabular}
{ c  ||  p{0.15cm}  p{0.15cm}  p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.25cm}|p{0.15cm}}
%\textbf{VOC 2007}
\textsc{IMGNET}
 &aero& bike&bird&boat&botl	&bus&car&cat&chr	&cow	&tab	&dog	&hse	&mbik	&pers	&plt	&shp	&sofa	&trn	&tv&mAP\\
\hline
\textbf{RR-RR}& 34.3& 34.6& 19.9& 17.1& 10.8& 30.0& 33.0& 18.4& 9.7& 13.7& 1.4& 17.6& 17.7& 34.7& 13.9& 11.8& 15.2& 12.7& 6.3& 26.0& 18.9 \\
\textbf{W-RR}&35.9 &23.3 &16.9 &15.0 &11.8 &24.9 &35.2 &20.9 &11.2 &15.5 &0.1 &15.9 &15.6 &28.7 &13.4 &8.9 &3.7 &10.3 &0.6 &28.8 &16.8 \\
\textbf{W-UG}&38.6 &32.5 &18.7 &14.1 &9.7 &21.2 &36.0 &9.9 &11.3 &13.6 &0.9 &15.7 &15.5 &32.3 &15.9 &9.9 &9.7 &19.9 &0.1 &17.4 &17.1 \\
\textbf{RR-UG}&26.4 &36.3 &9.5 &9.6 &9.4 &5.8 &24.9 &0.4 &1.2 &12.8 &4.7 &14.4 &9.2 &28.8 &11.7 &9.6 &0.7 &4.9 &0.1 &12.2 &11.6 \\
\textbf{RG-UG}&32.7 &34.5 &20.2 &14.6 &9.4 &7.5 &30.1 &12.1 &2.3 &14.6 &9.3 &15.2 &11.2 &30.2 &12.3 &11.4 &2.2 &9.9 &0.5 &13.1 &14.7 \\
\textbf{RG-RR}&26.4 &38.2 &21.0 &15.4 &12.1 &26.7 &34.5 &18.0 &8.8 &16.4 &0.4 &17.0 &20.9 &32.1 &11.0 &14.7 &18.4 &14.8 &6.7 &32.0 &19.3 \\
\end{tabular}
\end{center}
\caption{Detection results on the PASCAL VOC2007 test dataset. Each row is trained on different background and texture configuration of virtual data shown in the top table. In the middle table, the CNN is trained on ImageNet ILSVRC 1K classification data and finetuned on the PASCAL training data; in the bottom table, the network is not fine-tuned on PASCAL.}
\label{tab:color}
\vspace{-0.1in}
\end{table*}

\begin{figure*}[t]
\centering
%\includegraphics[width = 3in]{pos.jpg}
\includegraphics[width=0.49\linewidth]{neuron-tv.png}
\includegraphics[width=0.49\linewidth]{neuron-sheep.png}
%\includegraphics[width=0.49\linewidth]{A.png}
%\includegraphics[width=0.49\linewidth]{B.png}
%\includegraphics[width=0.49\linewidth]{C.png}
%\includegraphics[width=0.49\linewidth]{D.png}
%\includegraphics[width=0.49\linewidth]{E.png}
%\includegraphics[width=0.49\linewidth]{F.png}
%\includegraphics[width=0.49\linewidth]{faulty-A.png}
%\includegraphics[width=0.49\linewidth]{faulty-B.png}

%Kate: to save space just keep two of these for now
\caption{\textbf{Top 10 regions with strongest activations for 2 $pool_5$ units} using the method of~\cite{RCNN}. Overlay of the unit's receptive field is drawn in white and normalized activation value is shown in the upper-left corner. For each unit we show results on (top to bottom): real PASCAL images, RR-RR, W-RR, W-UG.}
\label{fig:pool5vis}
\end{figure*}

%\kate{add sentence to describe the pool5 visualization figure}
To better explore the CNN's invariance to color, texture and background, we visualize the patches which have the strongest activations for $pool_5$ units, as shown in Figure \ref{fig:pool5vis}.  The value in the receptive field's upper-left corner is normalized by dividing by max activation value over all units in a channel. The results are very interesting. The unit in the left subfigure fires on patches resembling tv-monitors in real images; when using our synthetic data, the unit still fires on tv-monitors even though the background and texture are removed. The unit on the right fires on white animals on green backgrounds in real and \textbf{RR-RR} images, and continues to fire on synthetic sheep with simulated texture, despite lack of green background. However, it fails on \textbf{W-UG} images, demonstrating its specificity to object color and texture.



\subsection{Synthetic Pose}

We also analyse the invariance of CNN features to 3D object pose. Through the successive operations of convolution and max-pooling, CNNs have a built-in invariance to translations and scale. Likewise, visualizations of learned filters at the early layers indicate a built-in invariance to local rotations. Thus while the CNN representation is invariant to slight translation, rotations and deformations, it remains unclear to what extent are CNN representation to large 3D rotations.

For this experiment, we fix the CAD models to three dominant poses: front-view, side-view and intra-view, as shown in Table~\ref{tab:diffpos}. We change the number of views used in each experiment, but keep the total number of synthetic training images (\textbf{RR-RR}) exactly the same, by generating random small perturbations (-15 to 15 degree) around the main view. Results indicate that for both networks adding side view to front view gives a boost, but improvement from adding the third view is marginal. We note that adding some views may even hurt performance (e.g., TV) as the PASCAL test set may not have objects in those views.

%\begin{figure*}[t]
%\centering
%%\includegraphics[width = 3in]{pos.jpg}
%\includegraphics[width=\linewidth]{virtual-views.png}
%\caption{Examples of CAD models views used in the pose invariance experiment. }
%\label{fig:CADpose}
%\end{figure*}

\begin{table*}[t]
\scriptsize  
\begin{center}
\includegraphics[width=0.8\linewidth]{virtual-views.png} \\
\begin{tabular}
%{c|| c c}
{c  ||  p{0.15cm}  p{0.15cm}  p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.25cm}|p{0.15cm}}
IMGNET &areo& bike&bird&boat&botl	&bus&car&cat&chr	&cow	&tab	&dog	&hse	&mbik	&pers	&plt	&shp	&sofa	&trn	&tv&mAP\\
\hline
\textbf{front}& 24.9& 38.7& 12.5& 9.3& 9.4& 18.8& 33.6& 13.8& 9.7& 12.5& 2.1& 18.0& 19.6& 27.8& 13.3& 7.5& 10.2& 9.6& 13.8& 28.8& 16.7\\
\textbf{front,side}& 24.3& 36.8& 19.0& 17.7& 11.9& 26.6& 36.0& 10.8& 9.7& 15.5& 0.9& 21.6& 21.1& 32.8& 14.2& 12.0& 14.3& 12.7& 10.1& 32.6& 19.0\\
\textbf{front,side,intra}& 33.1& 40.2& 19.4& 19.6& 12.4& 29.8& 35.3& 16.1& 5.2& 16.5& 0.9& 19.7& 19.0& 34.9& 15.8& 11.8& 19.7& 16.6& 14.3& 29.8& 20.5\\
\hline
\end{tabular}

\begin{tabular}
{c  ||  p{0.15cm}  p{0.15cm}  p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}  p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.15cm}p{0.15cm} p{0.15cm} p{0.25cm}|p{0.15cm}}
{PASC-FT} &aero& bike&bird&boat&botl	&bus&car&cat&chr	&cow	&tab	&dog	&hse	&mbik	&pers	&plt	&shp	&sofa	&trn	&tv&mAP\\
\hline
\textbf{front}& 41.8& 53.7& 14.5& 19.1& 11.6& 42.5& 40.4& 25.5& 9.9& 24.5& 0.2& 29.4& 37.4& 47.1& 14.0& 11.9& 18.9& 12.7& 22.6& 38.8& 25.8\\
\textbf{front,side}& 45.6& 50.2& 24.4& 28.8& 17.4& 51.9& 41.8& 24.5& 7.2& 27.9& 9.2& 23.1& 37.0& 51.3& 17.8& 13.2& 28.6& 18.9& 9.3& 37.8& 28.3\\
\textbf{front,side,intra}& 54.2& 55.5& 22.7& 27.0& 20.5& 52.6& 40.1& 26.8& 8.1& 27.3& 2.3& 30.6& 36.6& 53.3& 17.8& 14.2& 34.1& 26.4& 19.3& 37.5& 30.3\\
\end{tabular}
\end{center}
\caption{Results of training on different synthetic views. The CNN used in the top table is trained on ImageNet-1K classification, the CNN in the bottom table is also finetuned on PASCAL 2007 detection.}
\label{tab:diffpos}
\vspace{-0.1in}
\end{table*}

\subsection{Real Image Pose}

We also test view invariance on real images. We are interested here in objects whose frontal view presentation differs significantly (ex: the side-view of a horse vs a frontal view). To this end, we selected 12 categories from the PASCAL VOC training set which match this criteria. Held out categories included rotationally invariant objects such as bottles or tables. Next, we split the training data for these 12 categories to prominent side-view and front-view, as shown in Table~\ref{tab:realpose}.

%\kate{The text says we train only on one view, but the table used to say we train on all EXCEPT the one view. which is is? for now I changed table to be consistent}\xpeng{the table is right, we train on all view except that one view. When we talked about the experiments, we want to know what will happen if we remove one certain pose.}

We train classifiers exclusively by removing one view (say front-view) and test the resulting detector on the PASCAL VOC test set containing both side and front-views.We also compare with random view sampling. Results, shown in Table~\ref{tab:realpose}, point to important and surprising conclusions regarding the representational power of the CNN features. Note that mAP drops by less than $2\%$ when detectors exclusively trained  by removing either view are tested on the PASCAL VOC test set. Not only are those detectors never presented with the second view, but they are also trained with approximately half the data. While this invariance to large and complex pose changes may be explained by the fact the CNN model was itself trained with both views of the object present, and subsequently fine-tuned with both views again present, the level of invariance is nevertheless remarkable. In a last experiment, we reduce the fine-tuning training set by removing front-view objects, 
%this was confusing wrt table
%while training a classifier exclusively on side-view objects 
and note a larger mAP drop of $5$ points (8\%), but much less than one may expect. We conclude that, for both networks, the representation groups together multiple views of an object. %\kate{insert tSNE if available} \xpeng{on the way}

%\begin{figure*}[t]
%\centering
%%\includegraphics[width = 3in]{pos.jpg}
%\includegraphics[width=\linewidth]{pascal-views.png}
%\caption{Examples of poses labeled for PASCAL real image data. }
%\label{fig:pos}
%\end{figure*}


\begin{table*}[t]
\small
\begin{center}
\includegraphics[width=0.6\linewidth]{pascal-views.png} \\
\begin{tabular}
%{c|| c c}
{c |c ||  p{0.25cm}  p{0.25cm}  p{0.25cm}  p{0.25cm} p{0.25cm} p{0.25cm} p{0.25cm} p{0.25cm}  p{0.25cm} p{0.25cm} p{0.25cm} p{0.40cm} |p{0.35cm}}

Net & Views &aero& bike&bird&bus&car&cow	&dog	&hrs	&mbik	&shp	&trn	&tv&mAP\\
\hline
PASC-FT & \textbf{all}&64.2&69.7&	50&	62.6&	71&	58.5&	56.1&	60.6&	66.8&	52.8&	57.9&	64.7&	61.2\\
PASC-FT &\textbf{-random}& 62.1&70.3&49.7&61.1&70.2&54.7&55.4&61.7&67.4&55.7&57.9&64.2&60.9\\
PASC-FT &\textbf{-front}&61.7&67.3&45.1&58.6&70.9&56.1&55.1&	59.0&66.1&54.2&53.3&61.6&59.1\\
PASC-FT & \textbf{-side}&62.0&70.2&48.9&61.2&70.8&57.0&53.6&59.9&65.7&53.7&58.1&64.2&60.4\\

PASC-FT(-front) & \textbf{-front}	&59.7&63.1&42.7&55.3&64.9&54.4&54.0&56.1&64.2&55.1&47.4&60.1&56.4\\
\hline
\end{tabular}

%Kate: cut for space, can put back later
%\begin{tabular}
%{c ||  p{0.25cm}  p{0.25cm}  p{0.25cm}  p{0.25cm} p{0.25cm} p{0.25cm} p{0.25cm} p{0.25cm}  p{0.25cm} p{0.25cm} p{0.25cm} p{0.40cm} }
%View &aero& bike&bird&bus&car&cow	&dog	&hrs	&mbik	&shp	&trn	&tv\\
%\hline
%\textbf{No. total images} &331&418&599&272&1644&356&538&406&390&353&328&367\\
%\textbf{No. sideview} &111&115&191&62&529&102&97&103&90&103&105&70\\
%\textbf{No. frontview} &91&146&174&84&428&75&119&103&81&99&109&82\\
%\end{tabular}

\end{center}
\caption{Results of training on different real image views. '-' represent removing a certain view.
%The bottom table shows the number of training images in each condition. 
}
\label{tab:realpose}
\vspace{-0.1in}
\end{table*}


% We have carried out a set of experiments to study the effects of pose to RCNN. The experiments are shown in table [insert a table]. It shows that removing a certain pose from the SVM layer of RCNN model fine-tuned with both front-view images and side-view images, the mAP will only drop by 1 or 2 points. If RCNN model is only fine-tuned by images with front-view objects, the mAP will drop by 2 points if the SVM is still trained on both views, but will drop by 5 points if the SVM is also trained with only front-view objects.  

% The RCNN model is pre-trained on 1.2m class-labeled images from Image-net and 17 categories from PASCAL are already included in Image-net. The fact that the RCNN model has already seen both views while pre-training may partly explain why there is only a little drop when removing one view. 

% We have proposed an assumption that the deep features are invariant to pose by parts. Take two absolute different view-points of cars for example, one is absolute front-view and from this view, only the headlamp, front cover and cab are visible; the other is absolute side-view and only doors, wheels and windows are visible .If a CNN model is not pre-trained on cars and not fine-tuned on images with both views, it will take the cars with these two different views for different categories. The visualization of pool5 features shows that wheels are actually a distinguished part of a car and many neurons are fired on wheels. So it will be very interesting when it comes to an intra-view cars from which we can see a part of wheels, doors, windows and maybe headlamp. When the RCNN model is training only on the intro-view cars, it will probably still can find out the absolute side-view cars for they both have wheels and doors to fire the correspondent neurons.



%In preliminary experiments, we found that the information in the background of the object, i.e. its visual context, is also important. The visualization of pool5 features \kate{where is the figure??} shows that when the background changes, the same neuron can fire on different patterns. This is not surprising as the CNN is directly applied to the raw pixels. When the background changes, the appearance of edge areas of the object also changes. 
% It is also interesting that many neurons fired on background information. 

%I don't quite understand this point
%From the results of VCNN pipelines, we find that if the contour of the whole object is more distinguished from the background, the mAP is likely to be higher though from the visualization of pool5 units shows that many units are fired on the parts of an object. 

%Data generation method for our model is quite similar with that used in~\cite{BMVC}. The main differences are: 1) they used only 2 CAD models per category while we use more models to cover the intra-class variations; 2) we add real-image background and texture to virtual images in an attempt to make them more realistic.

% talk about the gap somewhre else
%Empirically, color, textures, shape and background information are all critical to CNN. Because the convolutional layers are directly applied to the raw pixels of an image, local patterns and intensity are decisive to which neural unit will fire. It is therefore unclear whether the gap between realistic images and non-photorealistic virtual images, which lack realistic color, textures, and background information will cause the CNN to fail to produce a useful representation.

\subsection{3D Shape}

%In \cite{BMVC},  only 2 models per category are used to align the Office dataset because the intra-class variation of Office dataset is small. But there are more refined categories for a certain categories in PASCAL. The authors of~\cite{xiang2014beyond} used around 9 CAD models to align the PASCAL detection dataset.

Finally, we experiment with reducing intra-class shape variation by using fewer CAD models per category. We otherwise use the same settings as in the \textbf{RR-RR} condition with PASC-FT. %\kate{double check,is this true? is no.images still 2K?}\xpeng{It's true, we have experiment on this, the total number is the same 2k}
 From our experiments, we find that the mAP decreases by about 5.5 points from 28.9\% to 23.53\% when using only a half of the 3D models. This shows a significant boost from adding more shape variation to the training data, indicating less invariance to this factor.







==> datageneration.tex <==
\section{Virtual data generation}
\label{datageneration}

Data generation method for our model is quite similar with that used in~\cite{BMVC}. The main differences are: 1) they used only 2 CAD models per category while we use more models to cover the intra-class variations; 2) we add real-image background and texture to virtual images in an attempt to make them more realistic.

The CAD models are downloaded from 3D Warehouse by searching for the name of 20 object categories in the PASCAL Dataset. For each category, about 25 models were downloaded. Original poses of some of the CAD models can be arbitrary, for example, upside-down chairs or slanted cars. We adjust the CAD models's pose manually to 3-4 poses that best represent intra-class pose variance for PASCAL objects. Then for each model pose we generate 1-2 virtual images to form a virtual training dataset. The final number of images in the virtual training dataset is 2,000, with 100 positive instance per each of 20 categories.

To investigate the importance of realistic backgrounds and object textures, we downloaded some real images for each category. When generating virtual images, we randomly select a background image from this pool to project to the image plane and a texture image to map onto the CAD model. We also tried different generation settings as shown in Table \ref{tab:datageneration}.

\begin{table*}[ht]

\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|}
\hline
NO. &\textbf {R-R} & \textbf{W-R}&\textbf{W-UG}  &\textbf{R-UG}&\textbf{RG-UG}&\textbf{RG-R}\\ 
\hline
BG & Real&White & White &Real&Real Gray&Real Gray\\
\hline
TX &Real & Real&Uni Gray&Uni Gray&Uni Gray&Real\\
\hline

Sample& \includegraphics[width=0.5in]{real_real.jpg}
&\includegraphics[width=0.5in]{white_real.jpg}
& \includegraphics[width=0.5in]{white_gray.jpg}
&\includegraphics[width=0.5in]{real_gray.jpg}
&\includegraphics[width=0.5in]{realgray_gray.jpg}
&\includegraphics[width=0.5in]{realgray_real.jpg}\\

\hline

\end{tabular}
\end{center}
\caption{Samples for different configuration of data generation. For background(BG), we have tried real images, white scene, and real gray images; and two types of texture, ie. real image texture and uniform gray.}
\label{tab:datageneration}


\end{table*}



==> images/approach.tex <==
\section{Virtual Data Generation}

Data generation method for our model is quite similar with that used in~\cite{bmvc}. The main differences are: 1) they used only 2 CAD models per category while we use more models to cover the intra-class variations; 2) we add real-image background and texture to virtual images in an attempt to make them more realistic.

The CAD models are downloaded from 3D Warehouse by searching for the name of 20 object categories in the PASCAL Dataset. For each category, about 25 models were downloaded. Original poses of some of the CAD models can be arbitrary, for example, upside-down chairs or slanted cars. We adjust the CAD models's pose manually to 3-4 poses that best represent intra-class pose variance for PASCAL objects. Then for each model pose we generate 1-2 virtual images to form a virtual training dataset. The final number of images in the virtual training dataset is 2,000, with 100 positive instance per each of 20 categories. \kate{how do we generate 2 images, what changes? and why not always 2?}

To investigate the importance of realistic backgrounds and object textures, we downloaded some real images for each category. When generating virtual images, we randomly select a background image from this pool to project to the image plane and a texture image to map onto the CAD model. We also tried different generation settings as shown in Table??.

\kate{[Insert a Table to clarify]}

\section{Exploring the Invariances of the CNN}

Before training our VCNN model, we design a series of experiments to evaluate how deviation of various image formation factors such as the color, texture, background and pose of an object from those found in real images influence CNN model's performance. Using computer graphics techqnies we can easily the factors mentioned above to investigate the CNN's invariance.

For each experiment below, we training only the output layer of the network, using deep features pre-trained on real images ad inputs.	

\subsection{Color, texture, background}

Empirically, color, textures, shape and background information are all critical to CNN. Because the convolutional layers are directly applied to the raw pixels of an image, local patterns and intensity are decisive to which neural unit will fire. It is therefore unclear whether the gap between realistic images and non-photorealistic virtual images, which lack realistic color, textures, and background information will cause the CNN to fail to produce a useful representation.

To get better training configuration for the VCNN, we have tried a batch of experiment configurations for background, color and texture for the virtual images. To better align to the real images, the features extracted by RCNN for the following experiments are fine-tuned by PASCAL 2007 train+val datasets. 

\kate{	[Figure to insert: pipeline]}
\kate{	[Table to insert:]}

\cite{bmvc} showed that for training a HOG template model on virtual data rendered from CAD models, rendering natural backgrounds and textures is not needed, white backgrounds and uniform gray textures can be used with similar results. Their claim is that a discriminative HOG-based classifier basically learns the ``outlines'' of the object shape, and discards everything else. The HOG model can arguably even learn from line drawings of the objects, although this remains to be proven experimentally.

Now, would that be the case for deep CNN models? Can you train a classifier using deep features on line drawings? The answer would seem to be no, because the deep layers capture not just shape outlines, but complex mid-level features such as faces, object parts and other patterns. However, we can show experimentally that again, learning from white background and uniform gray texture achieves similar performance as learning from natural backgrounds and realistic textures. At least this is the case when training only the output layer of the network, using deep features pre-trained on real images.	

\kate{move this to result section, instead explain the generated backgounds etc}


From the results of VCNN pipelines, we find that if the contour of the whole object is more distinguished from the background, the mAP is likely to be higher though from the visualization of pool5 units shows that many units are fired on the parts of an object. 

\subsection{Pose Variation}

From different viewpoints, the same object may have absolutely different presentations. Many works 
%[cite http://cvgl.stanford.edu/papers/3D%20generic%20object%20categorization_iccv07.pdf ] 
have focused on studying the effect of pose in detection tasks. Thanks to the pooling layers in the CNN, the deep features are kind of invariant to rotation and perspective transformation. But when the pictures of a certain object are taken from totally different views or the object is deformable, they could be totally different to computer. Take horses for example, the contour of prominent side-view horse is different from the horses from front-view.

In this experiment, we select 12 categories from PASCAL, for which the front-view and side-view are easy to distinguish. For other categories such as bottle and table, it's hard to define the side-view and front-view.

We split the training data for these 12 categories to prominent side-way and front-view, as showed by [insert a figure]. We have carried out a set of experiments to study the effects of pose to RCNN. The experiments are showed in table [insert a table]. It shows that removing a certain pose from the SVM layer of RCNN model fine-tuned with both front-view images and side-view images, the mAP will only drop by 1 or 2 points. If RCNN model is only fine-tuned by images with front-view objects, the mAP will drop by 2 points if the SVM is still trained on both views, but will drop by 5 points if the SVM is also trained with only front-view objects.  

The RCNN model is pre-trained on 1.2m class-labeled images from Image-net and 17 categories from PASCAL are already included in Image-net. The fact that the RCNN model has already seen both views while pre-training may partly explain why there is only a little drop when removing one view. 

We have proposed an assumption that the deep features are invariant to pose by parts. Take two absolute different view-points of cars for example, one is absolute front-view and from this view, only the headlamp, front cover and cab are visible; the other is absolute side-view and only doors, wheels and windows are visible .If a CNN model is not pre-trained on cars and not fine-tuned on images with both views, it will take the cars with these two different views for different categories. The visualization of pool5 features shows that wheels are actually a distinguished part of a car and many neurons are fired on wheels. So it will be very interesting when it comes to an intra-view cars from which we can see a part of wheels, doors, windows and maybe headlamp. When the RCNN model is training only on the intro-view cars, it will probably still can find out the absolute side-view cars for they both have wheels and doors to fire the correspondent neurons.

From this point, when training our VCNN model, we fix the CAD models to 3-4 prominent poses, and rotate the 3D model by a random angle from 0 to 20 degrees in each of the three axes.

\subsection{Variation in 3D Models}


In \cite{bmvc}, only 2 models per category are used to align the Office dataset because the intra-class variation of Office dataset is small. But there are more refined categories for a certain categories in PASCAL. The authors of~\cite{xiang2014beyond} used around 9 CAD models to align the PASCAL detection dataset. But from our experiments, we find that the mAP will decrease by about 5.5 points from 28.9\% to 23.53\% when using only a half number of the 3D models described in section 2.1. And it requires more 3D models for the deformable categories in PASCAL.

\kate{NEED TO PUT ALL ABOVE results NuMBers in tABLES}

%%%%%%%%%%%%%%%%%%%
\section{ Experiments}

Detectors based on deep CNNs, including OverFeat and RCNN, need a large quantity of real training images and a lot of manual annotation work. There are only 20 categories in PASCAL and 200 categories in the ImageNet detection dataset. For many novel categories, the training data is limited. 

\subsection{Data acquisition}

Through the detailed descriptions above and dense experiments on finding out what really matters to train a VCNN, we finally choose the virtual images with real-images background and real-images texture.  We find it's important to use this configuration because: 1). When the CNN learns distinguished features for one category, the information from background is also very important. From previous works on image classification, the CNN will mistake the truck in the snow for snow plough because the background for the snow plough category is critical. 2). Textures on object are also important because the CNN is operated on the raw pixels. 

Although the virtual dataset with white background and uniform gray texture can get a comparable mAP with virtual dataset with real-image background and real-image texture, the visualization of the positive training data shows that the white patch around the objects makes it harder to sample negative training data, under the schema of selective search.

\subsection{Results of experiments on color, texture, background}

The experiments indicate that the mAP is determined by how distinguished the object is from the background. When using the uniform gray texture and the white background, the mAP-30.14\% is comparable to the mAP-28.9\% from VCNN trained by virtual images with real-image background and real-image texture. And when using the non-colored real-gray background with colored real image texture on the target objects, the mAP is 31.18\%, 6-9 points higher than the performance of VCNN trained on virtual images with real-image background and uniform gray texture and VCNN trained on virtual images with real-gray background and uniform gray texture, in which the foreground images are not quite distinguished from the background.



\subsection{Results of Final VCNN Configuration}
\kate{not entirely happy with this title}

\kate{refer to results figure}
Our model obtains a mAP of 27.05\% on PASCAL detection test dataset with 2k virtual images. The pipeline of our model is similar to RCNN, with region proposal by selective search, similar CNN architecture designed by Krizhevsky et al [cite], and supervised pre-training. The difference is that, instead of depending on the manually annotated PASCAL trainval dataset, we use only 2k virtual images to fine-tune the pre-trained CNN and use the features extracted by the fine-tuned CNN to train the SVM. We strongly recommend our paper readers to refer RCNN for more details.

At test time, we run selective search on the test images to extracted around 2k region proposals and forward propagate each warped region proposal through VCNN to extract the feature using the Caffe [cite] implementation of CNN. Then using the corresponding SVM to score the 4096-dimensional feature vector. Then apply non-maximum suppression to all the scored proposals to reject a proposal if it has an IoU overlap with a higher score.

\kate{[Insert a pipeline here to show how it works]}
      
\kate{move to results} 
It’s often the truth that there are no annotated realistic images for a novel category.   When VCNN model is only pre-trained on Image-net, the mAP is 23.32\%.When the network is fine-tuned by Pascal trainval datasets, the AP goes to 28.9\%; when the network is fine-tuned on Image-net detection dataset with 200 categories, the AP is 27.24\%. 


\begin{table}[th]
\centering
\begin{tabular}{|l|l|l|c|}
\hline
Pre-train & Finetuning & SVM-Training & mAP \\ \hline
Imagenet 1.2m &
None  &
Virtual & 
23.32 \\ \hline
Imagenet 1.2m  &
Pascal  &
Virtual  &
28.9 \\ \hline
Imagenet 1.2m   &
Imagenet 200 &
Virtual &
27.24 \\ \hline
Imagenet 1.2m  &
virtual &
Virtual &
27.05 \\ \hline

\end{tabular}
\vspace{0.1in}
\caption{Effect of finetuning.}
\label{tab:nets}
\end{table}

We have also designed a set of experiments to simulate the situation that the number of realistic images is limited. Basically, for every category, we will randomly select 20(10, 5) positive training images to form datasets $R_{20}$ ($R_{10}$, $R_{5}$). The sizes of final datasets are 276(120, 73) because there are some images which contain two or more positive data. The size of virtual datasets (noted as $V_{2k}$) is still 2000. We use dataset $R_{x}$ (x=20,10,5) to train RCNN model, $R_{x}$+$V_{2k}$ to train our VCNN model, and $R_{x}$+$V_{2k}$ to train the Fast-Ada model. Due to the training data for RCNN is limited, the RCNN is only pre-trained on Image-net and not fine-tuned. The VCNN model is pre-trained on Image-net and fine-tuned by $V_{2k}$.

The result shows that when the number of training data is limited, VCNN will perform better than traditional RCNN for the lack of training data. The VCNN will also perform better than the Fast Adaptation method described in \cite{bmvc}.
 Refer to Table~\ref{tab:nets} and explain!



\begin{figure}[t]
\begin{center}
%   \includegraphics[width=\linewidth]{mainresult.png}
\end{center}
   \caption{\kate{TODO Comparison with RCNN and White-HOG method\cite{bmvc}}}
\label{fig:main}
\end{figure}



==> vcnn.tex <==

\section{Virtual Convolutional Neural Network for Object Detection}
\label{vcnn}
To summarize the conclusions from the previous section, we found that CNNs learn a significant amount of invariance to texture, color and pose, if trained (or fine-tuned) on the same task. If not trained on the task, however, the degree of invariance is lower. Therefore, when learning a detection model for a new category with no or limited labeled real data available, it is preferable to simulate these factors in the synthetic data.

Based on these findings, we propose an approach for using CNNs with CAD-generated virtual images, which we call the Virtual CNN (VCNN).
% for generating synthetic data for use with CNNs, the Virtual CNN. 
Our configuration uses all available 3D models and views, and selects a natural image background and real color image texture for each generated image (\textbf{RR-RR} in Table~\ref{tab:color}. We also propose to fine-tune the layers on the virtual data. 
Our VCNN model is similar to RCNN, with region proposals by selective search and supervised pre-training on ILSVRC. The difference is that, instead of depending on manually annotated real images, we use only the virtual images to fine-tune the pre-trained CNN, and use the features extracted by the fine-tuned VCNN to train the SVM detectors. 

%textbf{Data acquisition}
%
%Through the detailed descriptions above and dense experiments on finding out what really matters to train a VCNN, we finally choose the virtual images with real-images background and real-images texture.  


%The advantages of this configuration are as follows: 1) When the CNN learns distinguished features for one category, the information from background is also very important. From previous works on image classification, the CNN may mistake the truck in the snow for snow plough because the background for the snow plough category is critical. 2). Textures on object are also important because the CNN is operated on the raw pixels. 

We note that there may be other advantages to using realistic backgrounds. Visualizations of the positive training data show that white background around the objects makes it harder to sample negative training data via selective search, as most of the interesting regions are on the object.

%\subsection{Experiments}

%Our model obtains a mAP of 27.05\% on PASCAL detection test dataset with 2k virtual images. 
%At test time, we run selective search on the test images to extracted around 2k region proposals and forward propagate each warped region proposal through VCNN to extract the feature using the Caffe [cite] implementation of CNN. Then using the corresponding SVM to score the 4096-dimensional feature vector. Then apply non-maximum suppression to all the scored proposals to reject a proposal if it has an IoU overlap with a higher score.

%It is often the truth that there are no annotated realistic images for a novel category.   When VCNN model is only pre-trained on Image-net, the mAP is 22.05\%.When the network is fine-tuned by Pascal trainval datasets, the AP goes to 28.9\%; when the network is fine-tuned on Image-net detection dataset with 200 categories, the AP is 27.24\%. 

%\begin{table}[th]
%\centering
%\begin{tabular}{|l|l|l|c|}
%\hline
%Pre-train & Finetuning & SVM-Training & mAP \\ \hline
%Imagenet 1.2m &
%None  &
%Virtual & 
%22.05\\ \hline
%Imagenet 1.2m  &
%Pascal  &
%Virtual  &
%28.9 \\ \hline
%Imagenet 1.2m   &
%Imagenet 200 &
%Virtual &
%27.24 \\ \hline
%Imagenet 1.2m  &
%virtual &
%Virtual &
%27.05 \\ \hline
%
%\end{tabular}
%\vspace{0.1in}
%\caption{Effect of finetuning.}
%\label{tab:nets}
%\end{table}

\noindent\textbf{Learning novel categories.}
We present a set of experiments to simulate the situation where the number of labeled real images for a novel category is limited or zero. For every category, we randomly select 20 (10, 5) positive training images to form datasets $R_{20}$ ($R_{10}$, $R_{5}$). The sizes of final datasets are 276 (120, 73); note that there are some images which contain two or more positive bounding boxes. The size of the virtual dataset (noted as $V_{2k}$) is always 2000. Our VCNN is pre-trained on Imagenet ILSVRC (IMAGENET network) and fine-tuned on $V_{2k}$, then the SVMs are trained on both  $R_{x}$+$V_{2k}$.
We compare the two best configurations from Table~\ref{tab:color}, \textbf{RR-RR} and \textbf{RG-RR}. 

\noindent\textbf{Baselines.} We use datasets $R_{x}$ ($x=20,10,5$) to train the RCNN model, and $R_{x}$+$V_{2k}$ to train the Fast Adaptation method described in \cite{BMVC}. %Because we assume that real training data for RCNN is limited, 
The RCNN is pre-trained on Imagenet ILSVRC, however it is not fine-tuned on detection on $R_{5}$ and $R_{10}$ as data is very limited. 
%For comparison, we also propose a baseline in which the synthetic image dataset is \textbf{RG-RR}.% shown by green line in Figure \ref{results}.



%\kate{mention W-BG baseline}

\noindent\textbf{Results.} The results in Figure~\ref{results} show that when the number of real training images is limited, VCNN will perform better than traditional RCNN. The VCNN also significantly outperfoms the Fast-Adapt method, which is based on HOG features. We also confirm that our proposed \textbf{RR-RR} data synthesis methodology is better than not simulating background or texture. In partcular, fine-tuning on virtual \textbf{RR-RR} data boosts mAP from 18.9\% (Table~\ref{tab:color}) to 22\% without using any real training examples, and to 28\% with 5 real images per category, a 10\% absolute improvement over RCNN. We also notice that the results for \textbf{RG-RR} are much lower than \textbf{RR-RR}, which is not very surprising. Unlike \textbf{RR-RR}, \textbf{RG-RR} with selective search generates many sub-regions without color, and using these regions to fine-tune likely decreases the CNN's ability to recognize realistic color objects.

Note that the VCNN trained with 10 real images per category (200 total) is also using the approximately 900 real images of texture and background. However, this is still much fewer than the 15588 annotated bounding boxes in the PASCAL training set, and much easier to collect as only the texture images (about 130) need bounding box annotation. Yet the obtained 31\% mAP is comparable to the 33\% mAP achieved by the DPM (without context rescoring) trained on the full dataset. This speaks to the power of transferring deep representations and suggests that synthetic CAD data is a promising way to avoid tedious annotation for novel categories.

%9,963 total annotated images in pascal

\begin{figure}
\centering
\includegraphics[width=0.65\linewidth]{2.png}
\caption{Detection results of the proposed VCNN on PASCAL. When the real annotated images are limited or not available, eg. for a novel category, VCNN performs much better than RCNN and the Fast Adaptation method.}%\kate{fix zero-ex point for FastAdapt}}
\label{results}
\end{figure}


